Revisiting Email Spoofing Attacks

The email system is the central battleground against phishing and social engineering attacks, and yet email providers still face key challenges to authenticate incoming emails. As a result, attackers can apply spoofing techniques to impersonate a trusted entity to conduct highly deceptive phishing attacks. In this work, we study email spoofing to answer three key questions: (1) How do email providers detect and handle forged emails? (2) Under what conditions can forged emails penetrate the defense to reach user inbox? (3) Once the forged email gets in, how email providers warn users? Is the warning truly effective? We answer these questions through end-to-end measurements on 35 popular email providers (used by billions of users), and extensive user studies (N = 913) that consist of both simulated and real-world phishing experiments. We have four key findings. First, most popular email providers have the necessary protocols to detect spoofing, but still allow forged emails to get into user inbox (e.g., Yahoo Mail, iCloud, Gmail). Second, once a forged email gets in, most email providers have no warnings for users, particularly on mobile email apps. Some providers (e.g., Gmail Inbox) even have misleading UIs that make the forged email look authentic. Third, a few email providers (9/35) have implemented visual security cues for unverified emails, which demonstrate a positive impact to reduce risky user actions. Comparing simulated experiments with realistic phishing tests, we observe that the impact of security cue is less significant when users are caught off guard in the real-world setting.

==> Makefile <==
# $Id: Makefile,v 1.7 2014/06/28 01:18:01 Gang Exp $

PACKAGE=IEEEtran

LATEX=latex

BIBTEX=bibtex
BIBFILE=bibliography.bib wang.bib astro.bib
PAPER=email

TEXFILES = \
	email.tex \

#introduction.tex \
#	background.tex \
#	ui.tex \
#	top1m.tex \
#	user.tex \
#	email.tex \
#	related.tex \
#	conclusions.tex

PDF = ${TEXFILES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

$(PAPER).pdf: $(PAPER).tex

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

clean:
	rm -f *.dvi *.aux *.ps *~ *.log *.lot *.lof *.toc *.blg *.bbl *.pdf *.out
